LLM Self-Recognition: Steering and Retrieving Activation Signatures

Recent advances in interpretability suggest that large language models (LLMs) implicitly encode signals in their generated text that enable self-recognition of their outputs. We demonstrate that this capability is reliable, even in low-entropy scenarios, and that it can be amplified through targeted intervention. By steering the internal residual stream during generation with a random sparse vector, we create a detectable fingerprint that enables attribution of a given text to a specific LLM. This signal is recoverable from the activations of an LLM used as a detector, achieving over 98% accuracy across multiple detection settings while preserving the quality of generated text. As AI-generated content proliferates, this approach offers a practical alternative to traditional detectors by leveraging the model's natural representation structure for attribution rather than embedding a signal externally. Our contributions include: (i) establishing reliable self-recognition capabilities in LLMs, (ii) a simple steering mechanism enabling multi-LLM identification with no quality degradation, (iii) demonstrating that activation spaces contain exploitable structure for encoding signals without semantic interference.

==> Tables/cosine_similarity_classification_results.tex <==
\begin{table}[h]
\centering
\renewcommand{\arraystretch}{1.25}
\begin{tabular}{lccc}
\hline
\textbf{Evaluation} & \textbf{Group 1} & \textbf{Group 2} & \textbf{Overall} \\
\hline
\multicolumn{4}{l}{\textbf{Token-level classification}} \\
\quad Original      & 65.67\% & 58.45\% & 62.06\% \\
\quad Paraphrased   & 62.28\% & 58.49\% & 60.39\% \\
\hline
\multicolumn{4}{l}{\textbf{Sentence-level voting}} \\
\quad Original      & 87.55\% & 76.59\% & \textbf{82.07}\% \\
\quad Paraphrased   & 82.57\% & 75.79\% & \underline{79.18}\% \\
\hline
\multicolumn{4}{l}{\textbf{Cosine weighted sentence-level}} \\
\quad Original      & 89.21\% & 73.41\% & \underline{81.31}\% \\
\quad Paraphrased   & 84.23\% & 77.78\% & \textbf{81.01}\% \\
\hline
\end{tabular}
\caption{Classification accuracies across evaluation schemes, using only cosine similarity to the original steering vector.}
\end{table}

==> Texts/old_stuff_backup_just_in_case_you_know/2.Method.tex <==
\section{Method}

While an LLM is producing a new token, we can access its internal state and information flow during inference.
We can use this access either to gather the information or to learn recognition patterns.
Alternatively, we can use it to influence the model by adding information to the process.


%%%%%%%%%%%%%%%%%%%%%%%%%%
%%   Extraction method   %
%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Extracting the LLM's representation of a text}  \label{sec:gathering}

%\begin{itemize}
%    \item Goal: Extract a representation from the Upstream text. For classification.
%    \item How: Select a layer at which to take the intermediate representation
%    \item Extraction details (?): Averaging tokens to compress the representation.
%\end{itemize}

% Formal description of the extraction process.
Given a model $M$ with $L$ layers, let $l \in \{1, \ldots, L\}$ denote a specific layer and $\mathbf{x} = [x_1, x_2, \ldots, x_n]$ denote the input sequence of tokens. 

The representation extraction is formalized as:
\begin{equation}
\mathbf{r} = \text{Agr}\left(\mathbf{A}_l(x_0), \mathbf{A}_l(x_1), \ldots \mathbf{A}_l(x_n) \right)
\end{equation}

where $\mathbf{A}_l(x_i)$ is the intermediate activation at layer $l$ downstream from the token $x_i$, and $\text{Agr}$ denotes tokenwise averaging to produce the compressed representation $\mathbf{r} \in \mathbb{R}^d$.


%%%%%%%%%%%%%%%%%%%%%%%%
%%   Steering method   %
%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Steered LLM generation} \label{sec: steering}

%\begin{itemize}
%    \item Goal: Influence the downstream generated text
%    \item How: Add a vector to the representation before it goes to next layer.
%\end{itemize}

To steer the model according to a directive vector $\boldsymbol{v}$ by a given amplification coefficient $\alpha$, we simply proceed by adding the scaled vector to the intermediate activation at each token generation step:

\[ 
    \mathbf{A}_l(x_i) \leftarrow \mathbf{A}_l(x_i) + \alpha \boldsymbol{v}
\]


\subsection{Multi-bit watermarking parameterization}

%
The amplified self-recognition protocol, which enables us to distinguish text generated by different versions of the same LLM type, is as follows.
\begin{itemize}
    \item We start by generating $B$ random sparse vectors $\boldsymbol{v_1}, \boldsymbol{v_2}, \ldots, \boldsymbol{v_B}$ in the model's representation space $\mathbb{R}^d$. Each vector corresponds to a bit position in the watermark.
    \item During text generation, for each bit position $b$, if the bit to be encoded is 1, we add $\alpha \boldsymbol{v_b}$ to the intermediate activation at layer $l$; if the bit is 0, we do not modify the activation.
    \item After generation, to decode the watermark, we extract the representation $\mathbf{r}_t$ of the generated text $t$ as described in Section~\ref{sec:gathering}
    \item We then compute the dot product between $\mathbf{r}_t$ and each of the watermark vectors $\boldsymbol{v_b}$. If the dot product exceeds a predefined threshold $\tau$, we decode the corresponding bit as 1; otherwise, we decode it as 0.
\end{itemize}

The choice of parameters, such as the layer $l$, the amplification coefficient $\alpha$, the sparsity of the vectors, and the threshold $\tau$, is tuned via a grid search to achieve the same generation quality as the vanilla LLM while maximizing detection performance.


==> Texts/old_stuff_backup_just_in_case_you_know/old_abstract.tex <==
    % INTRO: WE NEED
    The rapid proliferation of AI-generated content raises safety concerns, as current watermarking techniques remain either insufficiently robust or too complex to deploy at scale. 
    % RECENTLY
    Meanwhile, recent advances in interpretability demonstrate that large language models (LLMs) implicitly encode a signal in their generated text that enables self-recognition of their outputs. 
    % WHAT WE PROPOSE
    We leverage this capability to propose a novel, minimally invasive method for identifying the LLM generating a given piece of text.
    % HOW IT WORKS
    With a random sparse steering in the internal residual stream, we amplify the natural fingerprint of the LLM in the generated text.
    This signal is then recoverable in the activations of an LLM used as detector on the generated text.
    % BENEFITS
    Our method encodes in the text a seamless signal, detectable with over $98\%$ accuracy at the cost of no quality loss across different LLMs. %and offers robustness toward paraphrasing.
    % CONTRIBUTIONS
    Our contributions include: 
    (i) we establish that LLMs exhibit a reliable self-recognition,
    (ii) a simple steering mechanism enabling multi-LLM identification, 
    (iii) new insights into activation engineering and it's intrinsic watermarking property.

